Probing LLM World Models: Enhancing Guesstimation with Wisdom of Crowds Decoding

Guesstimation -- the task of making approximate quantitative estimates about objects or events -- is a common real-world skill, yet remains underexplored in large language model (LLM) research. We introduce three guesstimation datasets: MARBLES, FUTURE, and ELECPRED, spanning physical estimation (e.g., how many marbles fit in a cup) to abstract predictions (e.g., the 2024 U.S. presidential election). Inspired by the social science concept of Wisdom of Crowds (WOC)- where the median of multiple estimates improves accuracy-we propose WOC decoding for LLMs. We replicate WOC effects in human participants and find that LLMs exhibit similar benefits: median aggregation across sampled responses consistently improves accuracy over greedy decoding, self-consistency decoding, and mean decoding. This suggests that LLMs encode a world model that supports approximate reasoning. Our results position guesstimation as a useful probe of LLM world knowledge and highlight WOC decoding as a strategy for enhancing LLM guesstimation performance on real-world tasks.

==> figures/diagram_prompts.tex <==
\begin{figure}[tb!] 
\centering
\caption{\sn{TODO}} 
\includegraphics[width=0.9\linewidth]{figures/diagram_prompts_fig.pdf}
% \vspace{-2mm}
\label{fig:diagram_prompts}
% \vspace{-4mm}
\end{figure}

